Applicability of machine learning in uncertainty quantification of turbulence models

White paper: The aim of this work is to apply and analyze machine learning methods for uncertainty quantification of turbulence models. In this work we investigate the classical and data-driven variants of the eigenspace perturbation method. This methodology is designed to estimate the uncertainties related to the shape of the modeled Reynolds stress tensor in the Navier-Stokes equations for Computational Fluid Dynamics (CFD). The underlying methodology is extended by adding a data-driven, physics-constrained machine learning approach in order to predict local perturbations of the Reynolds stress tensor. Using separated two-dimensional flows, we investigate the generalization properties of the machine learning models and shed a light on impacts of applying a data-driven extension.

==> WhitePaper_KucharczykThesis(4)_new/literatur.tex <==
\begin{thebibliography} {14}
 \bibitem{banerjee2007} \textsc{S. Banerjee, R. Krahl, F. Furst  and C. Zenger}, Presentation of anisotropy properties of turbulence, invariants versus
eigenvalue approaches, \textit{Journal of Turbulence} \textbf{8} (2007).
%\bibitem{blazek2005} \textsc{J. Blaszek}, \textit{Computational Fluid Dynamics: Principles and Applications 2nd. edn.}, Elsevier, Amsterdam (2005).
 %\bibitem{breiman2004} \textsc{L. Breiman}, Bagging predictors, \textit{Machine Learning} \textbf{24} (2004), 123--140.
  %\bibitem{breiman2001} \textsc{L. Breiman}, Random Forests, \textit{Machine Learning} \textbf{45} (2001), 5--32.
 \bibitem{breuer2009} \textsc{M. Breuer, N. Peller, C. Rapp and M. Manhart}, Flow over periodic hills – Numerical and experimental study in a wide
range of Reynolds numbers, \textit{Computers Fluids} \textbf{38} (2010), 433--457.
 %\bibitem{cook2019} \textsc{L. Cook, A. A. Mishra, J. Jarrett, K. Willcox and G. Iaccarino},ptimization ander turbulence model uncertainty for aerospace
%design, \textit{Physics of Fluids} \textbf{31} (2019), 105--111.
 %\bibitem{trace2022} \textsc{DLR, German Aerospace Center, Institute of Propulsion Technology}, \textsc{Trace} User Guide (2022), http://www.trace-portal.de/
%userguide/trace/index.html (visited in April 2022).
 \bibitem{duraisamy2019} \textsc{K. Duraisamy, G. Iaccarino and H. Xiao}, \mbox{Turbulence Modeling in the} Age of Data, \textit{Annual Review of Fluid Mechanics} \textbf{51} (2019), 357--377.
 %\bibitem{eidi2022} \textsc{A. Eidi, N. Zehtabiyan-Rezaie, R. Ghiassi, X. Yang and M. Abkar}, Data-driven quantification of model-form uncertainty in Reynolds-averaged simulations of wind farms, arXiv:2205.14221 (2022), https://arxiv.org/abs/2205.14221.
 \bibitem{emory_diss} \textsc{M. Emory}, Estimating model-form uncertainty in Reynolds-averaged NavierStokes closures,  Ph.D. Thesis, Stanford University, Stanford (2014).
\bibitem{emory2013} \textsc{M. Emory, J. Larsson and G. Iaccarino}, Modeling of structural uncertainties in Reynolds-averaged Navier-Stokes closures, \textit{Physics of Fluids} \textbf{25}: 110822 (2013).
%\bibitem{geron2019} \textsc{A. Géron}, \textit{Hands-On Machine Learning with Scikit-Learn, Keras, and TensorFlow 2nd edn.}, O'Reilly Media, Sebastopol (2019).
%\bibitem{hirsch1990} \textsc{C. Hirsch}, \textit{Numerical Computation of Internal and External Flows – Computational
%Methods for Inviscid and Viscous Flows 1st. edn.}, Wiley, Brüssel (1990).
\bibitem{heyse2021} \textsc{J. Heyse, A. A. Mishra and G. Iaccarino}, Estimating RANS model uncertainty using machine learning, \textit{Journal of the Global
Power and Propulsion Society} (2021), 1--14.
\bibitem{iaccarino2017} \textsc{G. Iaccarino, A. A. Mishra and S. Ghili}, Eigenspace perturbations for uncertainity estimation of single-point turbulence closures, \textit{Physical Review Fluids} \textbf{2} (2017).
\bibitem{kucharczyk} \textsc{K. Kucharczyk}, Anwendbarkeit von Machine Learning in der Unsicherheitsquantifizierung von Turbulenzmodellen, \textit{Master's thesis, University of Cologne, German Aerospace Cenetr} (2022).
\bibitem{laval2011} \textsc{J. Laval and M. Marquillie}, Direct Numerical Simulations of Converging–Diverging Channel Flow, \textit{Progress in Wall Turbulence: anderstanding and Modeling. ERCOFTAC Series} \textbf{14} (2011), 203--209, Springer-Verlag, Berlin.
\bibitem{lee2015} \textsc{M. Lee and R. Moser}, Direct numerical simulation of turbulent channel flow up to $Re_\tau \approx 5200$, \textit{Journal of Fluid
Mechanics} \textbf{774} (2015), 395--415.
%\bibitem{ling2016} \textsc{J. Ling, R. E. Jones and J. Templeton}, Machine learning strategies for systems with invariance properties, \textit{J. Comput. Phys.} \textbf{318} (2016), 22--35.
%\bibitem{lumley1979} \textsc{J. L. Lumley}, Computational modeling of turbulent flows, \textit{Advances in Applied Mechanics} \textbf{18} (1979), 123--176.
%\bibitem{lumley1977} \textsc{J. L. Lumley and G. Newman}, The return to isotropy of homogenous turbulence, \textit{Journal of Fluid Mechanics} \textbf{82} (1977), 161--178.
%\bibitem{matha2021} \textsc{M. Matha and C. Morsbach}, Extending turbulence model uncertainty quantification using machine learning, \textit{NeurIPS -
%Thirty-fifth Conference on Neural Information Processing Systems | Workshop on Machine %Learning and the Physical Sciences} (2021).
\bibitem{matha2022} \textsc{M. Matha, K. Kucharczyk and C. Morsbach}, Assessment of data-driven Reynolds stress tensor perturbations for uncertainty quantification of RANS turbulence models, \textit{AIAA Aviation Forum 2022} (2022).
\bibitem{matha2022CF} \textsc{M. Matha, K. Kucharczyk and C. Morsbach}, Evaluation of physics constrained data-driven methods for turbulence model uncertainty quantification, \textit{Preprint, under Review} (2022).
\bibitem{mishra2018} \textsc{A. A. Mishra, J. Mukhopadhaya, G. Iaccarino and J. Alonso}, An uncertainty estimation module for turbulence model
predictions in SU2, \textit{AIAA Journal} \textbf{57} (2018).
%\bibitem{mishra2019} \textsc{A. A. Mishra and G. Iaccarino}, Theoretical analysis of tensor perturbations for uncertainty quantification of Reynolds averaged and subgrid scale closures, \textit{Physics of Fluids} \textbf{31} (2019), 75--101.
%\bibitem{mishra2020} \textsc{A. A. Mishra, J. Mukhopadhaya,J. Alonso, and G.  Iaccarino}, Design exploration and optimization ander uncertainty, \textit{Physics of Fluids} \textbf{32} (2020), 85--106.
\bibitem{menter2003} \textsc{F. Menter, M. Kuntz and R. Langtry}, Ten years of industrial experience with the SST turbulence model, \textit{Heat and Mass Transfer} \textbf{4} (2003).
%\bibitem{morsbach2017} \textsc{C. Morsbach}, Reynolds Stress Modelling for Turbomachinery Flow Applications, Ph.D. Thesis, Teschnische Universität Darmstadt, Darmstadt (2017).
%\bibitem{nasa2022} \textsc{NASA, National Acronautics and Space Administration}, Turbulence modeling resource database, https://turbmodels.larc.nasa.gov/index.html (aufgerufen im April 2022).
\bibitem{pedregosa2011} \textsc{F. Pedregosa et al.}, Scikit-learn: Machine Learning in Python, \textit{Journal of Machine Learning Research} \textbf{12} (2011), 2825--2830.
%\bibitem{pope2000} \textsc{S. Pope}, \textit{Turbulent Flows}, Cambridge University Press, Cambridge (2000).
%\bibitem{scott2015} \textsc{D. Scott}, \textit{Multivariate Density
%Estimation: Theory, Practice, and Visualization: Second Edition}, Wiley, Brüssel (2015).
\bibitem{rossi2006} \textsc{R. Rossi}, Passive scalar transport in turbulent flows over a wavy wall,  Ph.D. Thesis,  Università degli Studi di Bologna, Bologna (2008).
\bibitem{scipy2020} \textsc{P. Virtanen et al.}, SciPy 1.0: Fandamental Algorithms for Scientific Computing in Python, \textit{Nature Methods} \textbf{17} (2020), 261--272.
%\bibitem{wilcox_model} \textsc{C. D. Wilcox}, Reassessment of the scale-determining equation for advanced turbulence models, \textit{AIAA Journal} \textbf{26} (1998), 1299--1310.
%\bibitem{wilcox2006} \textsc{C. D. Wilcox}, \textit{Turbulence Modeling for CFD 3rd edn.}, DCW Industries, La Cañada, USA (2006).
%\bibitem{wang2018} \textsc{J. Wang, J. Wu, J. Ling, G. Iaccarino and H. Xiao}, A Comprehensive Physics-Informed Machine Learning Framework
%for Predictive Turbulence Modeling, arXiv:1701.07102 (2018), https://arxiv.org/abs/1701.07102.
%\bibitem{wu2017} \textsc{J. Wu, J. Wang, H. Xiao and J. Ling}, A Priori Assessment of Prediction Confidence for Data-Driven Turbulence
%Modeling , \textit{Flow, Turbulence and Combustion} \textbf{99} (2017), 25--46.
%\bibitem{wu2018} \textsc{J. Wu, H. Xiao and E. Paterson}, Physics-Informed Machine Learning Approach for Augmenting
\bibitem{zang2002} \textsc{T. A. Zang, M. J. Hemsch, M. W. Hilburger, S. P. Kenny, J. M. Luckring,
P. Maghami, S. L. Padula and W. J. Stroud}, Needs and opportunities for
uncertainty-based multidisciplinary design methods for aerospace vehicles, \textit{Technical Report No. NASA/TM-2002-211462}, National Aeronautics and Space
Administration, Langley Research Center, 2002.
Turbulence Models: A Comprehensive Framework, \textit{Physical Review Fluids} \textbf{3}: 074602 (2018).
\end{thebibliography}




